funcX: Federated Function as a Service for Science

funcX is a distributed function as a service (FaaS) platform that enables flexible, scalable, and high performance remote function execution. Unlike centralized FaaS systems, funcX decouples the cloud-hosted management functionality from the edge-hosted execution functionality. funcX's endpoint software can be deployed, by users or administrators, on arbitrary laptops, clouds, clusters, and supercomputers, in effect turning them into function serving systems. funcX's cloud-hosted service provides a single location for registering, sharing, and managing both functions and endpoints. It allows for transparent, secure, and reliable function execution across the federated ecosystem of endpoints--enabling users to route functions to endpoints based on specific needs. funcX uses containers (e.g., Docker, Singularity, and Shifter) to provide common execution environments across endpoints. funcX implements various container management strategies to execute functions with high performance and efficiency on diverse funcX endpoints. funcX also integrates with an in-memory data store and Globus for managing data that may span endpoints. We motivate the need for funcX, present our prototype design and implementation, and demonstrate, via experiments on two supercomputers, that funcX can scale to more than 130 000 concurrent workers. We show that funcX's container warming-aware routing algorithm can reduce the completion time for 3000 functions by up to 61% compared to a randomized algorithm and the in-memory data store can speed up data transfers by up to 3x compared to a shared file system.

==> requirements.tex <==
\section{Requirements} \label{sec:requirements}

Our work is guided by the unique requirements of FaaS in science. 
To illustrate these requirements we present six representative case studies:
scalable metadata extraction, machine learning inference as a service, synchrotron serial crystallography, neuroscience, correlation spectroscopy, and high energy physics.  
\figurename~\ref{fig:use-cases} shows function execution time distributions for each case study. 
These short duration tasks exemplify opportunities for FaaS in science. 
We summarize by highlighting requirements for FaaS in science.


\begin{figure}[ht]
  \includegraphics[width=1\columnwidth,trim=0.08in 0.1in 0.08in 0.1in,clip]{Figures/use-cases}
    \vspace{-0.15in}
  \caption{Distribution of latencies for 100 function calls, for each of the six case studies described in the text.
\label{fig:use-cases}
  \vspace{-0.1in}
}
\end{figure}

\textbf{Metadata extraction:}
The effects of high-velocity data expansion are making it increasingly
difficult to organize, discover, and manage data. 
Edge file systems and data
repositories now store petabytes of data
which are created and modified at an alarming rate~\cite{paul17monitoring}.
\xtract{}~\cite{skluzacek19serverless} 
is a distributed metadata extraction system
that applies a set of
general and specialized metadata extractors, such as those for identifying topics in text, computing aggregate values from tables, and recognizing locations in maps. 
To reduce data transfer costs, \xtract{} executes extractors ``near'' to
data, by pushing extraction tasks to the edge. Extractors are implemented
as Python functions, with various dependencies, and each extractor typically executes for between 3 milliseconds and 15 seconds.


\textbf{Machine learning inference:}
\dlhub{}~\cite{chard19dlhub} 
is a service that supports ML model publication 
and on-demand inference. 
Users deposit ML models, implemented as functions with a set of
dependencies, in the \dlhub{} catalog
by uploading the raw model (e.g., PyTorch, TensorFlow) and model 
state (e.g., training data, hyperparameters).
\dlhub{} uses this information to dynamically create a container for the model using repo2docker~\cite{repo2docker} that contains all model dependencies and necessary model
state.
Other users may then invoke the model through \dlhub{} on arbitrary input
data. \dlhub{} currently includes more than one hundred published models, 
many of which have requirements for specific ML toolkits and execute
more efficiently on GPUs and accelerators. 
\figurename~\ref{fig:use-cases} shows the execution time when invoking the 
MNIST digit identification model. Other \dlhub{} models execute for between seconds and
several minutes. 

\textbf{Synchrotron Serial Crystallography (SSX)} %is a new technique that
is an emerging method for imaging small crystal samples 1--2 orders of magnitude faster than other methods. 
To keep pace with the increased data production, SSX researchers require automated 
approaches that can process the resulting data with great rapidity:
for example, to count the \emph{bright spots} in an image 
(``stills processing'') within seconds, both for quality control 
and as a first step in structure determination. The DIALS~\cite{waterman2013dials} crystallography processing tools are implemented
as Python functions that execute for 
1--2 seconds per sample. 
Analyzing large datasets requires HPC resources to derive crystal structures
in a timely manner.


\textbf{Quantitative Neurocartography} and connectomics map the 
neurological connections in the brain---a compute- and data-intensive process 
that requires processing \textasciitilde 20GB every minute during experiments.
Researchers apply automated workflows %are used 
to perform quality control on raw images (to validate that the instrument
and sample are correctly configured), apply ML models
to detect image centers for subsequent reconstruction, and generate
preview images to guide positioning. Each of these steps is implemented
as a function that can be executed sequentially with some data exchange
between steps. However, given the significant data sizes, researchers typically
rely on HPC resources and are subject to scheduling delays. 


\textbf{Real-time data analysis in High Energy Physics (HEP)}:
The traditional HEP analysis model uses successive processing steps to reduce the initial dataset (typically, 100s of PB) to a size that permits real-time analysis. This iterative approach requires significant computation time and storage of large intermediate datasets, and may take weeks or months to complete. Low-latency, query-based analysis strategies~\cite{pivarski2017} are being developed to enable real-time analysis
using native operations on hierarchically nested, columnar data. 
Such queries are well-suited to FaaS. % processing using \name{}. 
To enable interactive analysis, for example as a physicist engages in real-time analysis of several billion particle collision events, successive compiled functions, each running for seconds, need to be dispatched to the data. Analysis needs require sporadic (and primarily remote) invocation, and compute needs increase as new data are collected.


\textbf{X-ray Photon Correlation Spectroscopy (XPCS)} 
is an experimental technique used %at Argonne's Advanced Photon Source
to study the dynamics in materials at nanoscale by identifying correlations in 
time series of area detector images. 
This process involves analyzing the pixel-by-pixel correlations 
for different time intervals. 
The detector acquires megapixel frames at 60 Hz (\textasciitilde 120 MB/sec). 
Computing correlations at these data rates is a challenge that requires HPC resources but also rapid response time. Image processing functions, such as XPCS-eigen's corr function,
execute for approximately 50 seconds, and images can be processed in parallel.


\textbf{Requirements for FaaS in science:}
The case studies illuminate benefits of 
FaaS approaches (e.g., decomposition, abstraction, 
flexibility, scalability, reliability), but also
elucidate requirements unmet by existing FaaS solutions: 

\begin{itemize} %[leftmargin=*]
    \item \textbf{Specialized compute:} functions may require HPC-scale and/or specialized and heterogeneous resources (e.g., GPUs).   
    \item \textbf{Distribution:} functions may need to execute near to data and/or on a specialized computer. 
  	\item \textbf{Dependencies:} functions often require specific libraries and user-specified dependencies.
	\item \textbf{Data:} functions analyze both small and large data, stored in various locations and formats, and accessible via different methods (e.g., Globus~\cite{chard14efficient}).
    \item \textbf{Authentication:} institutional identities and specialized security models are used to access data and compute resources.
    \item \textbf{State:} functions may be connected and share state (e.g., files or database connections) to decrease overheads. 
    \item \textbf{Latency:} functions may be used in online (e.g., experiment steering) and interactive environments (e.g., Jupyter notebooks) that require rapid response. 
    \item \textbf{Research CI:} resources offer batch scheduler interfaces (with long delays, periodic downtimes, proprietary interfaces) and specialized container technology (e.g., Singularity, Shifter) that make it challenging to provide common execution interfaces, elasticity, and fault tolerance. 
    \item \textbf{Billing:} research CI use allocation-based usage models.
\end{itemize}




==> survey-long.tex <==
\section{A Brief Survey of FaaS}\label{sec:survey}

\kyle{Need to focus more on differences: distributed/multi-site execution, reliable execution on remote EPs, different resource providers, function targeting specific resource (e.g., endpoint X), we can use accelerators, data, scale (I expect the others do not scale that far).}
\kyle{Existing systems designed for kubernetes where you get auto responses, here we had
to do a lot to work with batch systems, provision nodes, scale nodes, deal with unreliability and unknown SLAs}

FaaS platforms have proved wildly successful in industry as a way
to reduce costs and the need to manage infrastructure.
Here we present a brief survey of FaaS platforms, summarized in \tablename{~\ref{tab:survey}}. 
We broadly categorize platforms as \emph{commercial}, \emph{open source}, or \emph{academic}.
%and further compare them based on the following categories.

%\begin{itemize}
% \item \textbf{Languages:} The programming languages that can be used to define functions.
% \item \textbf{Infrastructure:} Where the FaaS platform is deployed and where functions are executed, e.g., cloud, Kubernetes.
% \item \textbf{Virtualization:} The virtualization technology used to isolate and deploy functions.
% \item \textbf{Triggers:} How functions are invoked and whether specific event sources are supported.
% \item \textbf{Walltime:} How long functions are permitted to execute.
% \item \textbf{Billing:} What billing models are used to recoup costs.
%\end{itemize}
% RC: Trimming this to useful columns (infra, virt, walltime) and decided we don't need this list. Do we need others? Perhaps we don't even need a table wiht just 3 columns?

\definecolor{Gray}{gray}{0.9}
\newcolumntype{a}{>{\columncolor{Gray}}c}

\begin{table*}[]
\caption{Taxonomic survey of common FaaS platforms.} \label{tab:survey}

\vspace{-1ex}

%\footnotesize
%\begin{tabular}{|p{1.8cm}|p{2.7cm}|p{2.5cm}|p{2cm}|p{1.7cm}|p{1.6cm}|p{2cm}|}
%\hline
%\textbf{} & \textbf{Function Language} & \textbf{Intended Infrastructure} & \textbf{Virtualization} & \textbf{Triggers} %& \textbf{Maximum Walltime (s)} & \textbf{Billing} \\ \hline
%\textbf{Amazon Lambda} & C\#, Go, Java, Powershell, Ruby, Python, Node.js & Public cloud, Edge (Greengrass) & %Firecracker (KVM) &  HTTP, AWS services & 900 & Requests, runtime, memory \\ \hline
%\textbf{Google Cloud Functions} & BASH, Go, Node.js, Python & Public cloud & Undefined & HTTP, Pub/Sub, storage & 540 %&Requests, runtime, memory \\ \hline
%\textbf{Azure \newline Functions} & C\#, F\#, Java, Python, JavaScript & Public cloud, local & OS images & HTTP, APIM, %MS services &600 & Requests, runtime, SLA \\ \hline
%\textbf{OpenWhisk} & Ballerina, Go, Java, Node.js, Python & Kubernetes, Private cloud, Public cloud & Docker & HTTP, IBM %Cloud, OW-CLI & 300 & IBM Cloud: Requests, runtime Local: NA \\ \hline
%\textbf{Kubeless} & Node.js, Python .NET, Ruby Ballerina, PHP & Kubernetes & Docker & HTTP, scheduled, Pub/Sub & %Undefined & NA \\ \hline 
%\textbf{SAND} & C, Go, Java, Node.js, Python & Public cloud, Private cloud & Docker & HTTP, Internal event & Undefined & %Triggers \\ \hline
%\textbf{Fn} & Go, Java, Ruby, Node.js, Python &  Public cloud, Kubernetes & Docker & HTTP, direct trigger & 300 & NA \\ %\hline
%\textbf{Abaco} & Container & TACC clusters & Docker &  HTTP & Undefined & Undefined \\ \hline
%\rowcolor[HTML]{C0C0C0} 
%\textbf{\name{}} & Python & Local, clouds (AWS, Azure, GCP), clusters (e.g., Cobalt, Slurm, Torque/PBS), supercomputers %& Singularity, Shifter, Docker & HTTP, Globus Automate & No limit & HPC SUs, cloud credits. Local: NA \\ \hline
%\end{tabular}
%\end{table*}


\footnotesize
\begin{tabular}{|p{2.7cm}|p{4.5cm}|p{2.7cm}|p{2.3cm}|}
\hline
\textbf{} & \textbf{Intended Infrastructure} & \textbf{Virtualization} & \textbf{Max Walltime (s)} \\ \hline
\textbf{Amazon Lambda} & Public cloud, Edge (Greengrass) & Firecracker (KVM) &  900 \\ \hline
\textbf{Google Cloud Functions} & Public cloud & Undefined & 540 \\ \hline
\textbf{Azure Functions} & Public cloud, local & OS images & 600 \\ \hline
\textbf{OpenWhisk} & Kubernetes, Private cloud, Public cloud & Docker & 300 \\ \hline
\textbf{Kubeless} & Kubernetes & Docker & Undefined \\ \hline 
\textbf{SAND} & Public cloud, Private cloud & Docker & Undefined \\ \hline
\textbf{Fn} &  Public cloud, Kubernetes & Docker & 300 \\ \hline
\textbf{Abaco} & TACC clusters & Docker & Undefined \\ \hline
\rowcolor[HTML]{D0D0D0} 
\textbf{\name{}} & Local, clouds (AWS, Azure, GCP), clusters (e.g., Cobalt, Slurm, Torque/PBS), supercomputers & Singularity, Shifter, Docker & No limit \\ \hline
\end{tabular}
\end{table*}

\subsection{Commercial Platforms}
Most commercial cloud providers offer FaaS capabilities.
Here we compare three 
platforms offered by Amazon, Microsoft, and Google. 

\emph{Amazon Lambda}~\cite{AmazonLambda} pioneered the FaaS paradigm in 2014 and has since
be used in many 
industry~\cite{netflixlambda} and academic~\cite{chard17ripple} use cases. Lambda is a hosted service
that supports a multitude of function languages and trigger sources (Web interface, CLI, SDK, and other AWS services). 
Tight integration with the wider AWS ecosystem means Lambda functions can be associated with triggers from other AWS services, such as CloudWatch, S3, API gateways, SQS queues, and Step Functions. Functions are billed based on their memory allocation and 
for every 100ms execution time. Once defined, Lambda uses a custom virtualization technology built on KVM, called Firecracker to create lightweight micro-virtual machines. These microVMs then persist in a \textit{warmed} state for five minutes and continue to serve requests. 
While Lambda is provided as a hosted service, functions can be deployed locally or to edge devices 
via the Greengrass~\cite{greengrass} IoT platform. 

\emph{Google Cloud Functions}~\cite{googlecloudfunctions} is differentiated by its tight coupling to Google Cloud Storage, Firebase mobile backends, and custom IoT configurations via Google's globally distributed message bus (Cloud Pub/Sub).
Like Lambda, Google Cloud Functions also support triggers from arbitrary HTTP webhooks. 
Further, users can trigger functions through a number of third party systems including 
GitHub, Slack, and Stripe. 
While Google Cloud functions apply a similar pricing model to Lambda, the model is slightly more expensive
for high-volume, less computationally intensive tasks as Lambda has lower per-request costs after the first two million invocations (with similar compute duration costs). 

\emph{Azure Functions}~\cite{azureFunctions} allow users to create functions in a native language through either the Web interface or the CLI. Functions are packaged and may be tested locally using a local web service before being uploaded to the Azure platform.
Azure functions integrate with other Azure products through triggers. 
Triggers are provided from CosmosDB, Blob storage, and Azure storage queues, in addition to custom HTTP and time-based triggers. Azure price-matches AWS for compute and storage (as of November 2018).


\subsection{Open Source Platforms}
Open FaaS platforms resolve two of the key challenges to using FaaS for scientific workloads: they 
can be deployed on-premise and can be customized to meet the requirements of data-intensive 
workloads without any pricing models.

\emph{Apache OpenWhisk}~\cite{openwhisk} is the most well-known open source FaaS platform. OpenWhisk is the basis of IBM Cloud Functions~\cite{IBMCloudFunctions}. OpenWhisk clearly defines an event-based programming model, consisting of \emph{Actions} which are stateless, runnable functions, \emph{Triggers} which are the types of events OpenWhisk may track, and \emph{Rules} which associate one trigger with one action. OpenWhisk can be deployed locally as a service using a Kubernetes cluster. However, deploying OpenWhisk is non-trivial, requiring installation of dependencies and administrator access to the cluster. 

\emph{Fn}~\cite{Fn} is a powerful open-source software from Oracle that can be deployed on any Linux-based compute resource having administrator access to run Docker containers. Applications---or groups of functions---allow users to logically group functions to build runtime utilities (e.g.,
dependency downloads in custom Docker containers) and other resources (e.g.,
a trained machine learning model file) to support functions in the group. Moreover, Fn supports fine-grained logging and metrics, and is one of few open source FaaS platforms deployable on Windows. Fn can be deployed locally or on a Kubernetes cluster. In our experience, one can deploy a fully-functional Fn server in minutes.


\emph{Kubeless}~\cite{Kubeless} is a native 
Kubernetes FaaS platform that takes advantage of built-in 
Kubernetes primitives. Kubeless uses Apache Kafka for messaging, provides a CLI that mirrors that of AWS Lambda, and supports fine-grained monitoring. Users can invoke functions via the CLI, HTTP, and via a Pub/Sub mechanism. Like Fn, Kubeless allows users to define function groups that share resources.  Like OpenWhisk, Kubeless is reliant on Kubernetes and cannot be deployed on other resources.

\subsection{Academic Platforms}

The success of FaaS in industry has spurred academic exploration of FaaS. Two
systems that have resulted from that work are SAND~\cite{akkus2018sand} and Actor Based Co(mputing)ntainers (Abaco)~\cite{stubbs2017containers}.

\emph{SAND}~\cite{akkus2018sand} is a lightweight, low-latency FaaS platform from Nokia Labs that provides application-level sandboxing and a hierarchical message bus. The authors state that they achieve a 43\% speedup and a 22x latency reduction over Apache OpenWhisk 
in commonly-used image processing applications.
Further, SAND provides support for function or \textit{grain} chaining via user-submitted workflows. At the time of their writing, it appears that SAND does not support multi-tenancy, only having isolation at the application level.
SAND is closed source and as far as we know cannot be downloaded and installed locally.


\emph{Abaco}~\cite{stubbs2017containers} supports functions written in a wide range of programming languages and supports automatic scaling. Abaco implements the Actor model in which an \textit{actor} is an Abaco runtime mapped to a specific Docker image. Each actor executes in response to messages posted to its \textit{inbox}. Moreover, Abaco provides fine-grained monitoring of container, state, and execution events and statistics. Abaco is deployable via Docker Compose. 


\subsection{Summary of FaaS}
Commercial cloud providers implement high performance and reliable FaaS models 
that are used by huge numbers of users. However, for science use cases they 
are unable to make use of existing infrastructure, they do not integrate
with the science ecosystem (e.g., in terms of data and authentication models), 
and they can be costly. 

Open source and academic frameworks support on-premise deployments and can be 
configured to address a range of use cases. However, each of the systems surveyed
is Docker-based and therefore requires administrator privileges to be deployed 
on external systems. Furthermore, the reliance on Docker prohibits use in 
most computing centers which instead support user space containers. 
In most cases, these systems have been implemented to rely on Kubernetes (or other
container orchestration models such as Mesos and Openshift) which means
they cannot be adapted to existing HPC and HTC environments. 

\name{} provides a scalable, low-latency 
FaaS platform that can be applied to existing HPC resources with minimal effort. It employs user-space
containers to isolate and execute functions, avoiding the security concerns prohibiting other FaaS
platforms from being used. Finally, it provides an intuitive interface for executing scientific
workloads and includes a number of performance optimizations to support broad scientific use cases.


\subsection{Other Related Approaches}
FaaS builds upon a large amount of related work including
in Grid and cloud computing, container orchestration, and analysis systems. 
Grid computing~\cite{Foster2001} laid the foundation for 
remote, federated computations, most often applying 
federated batch submission~\cite{krauter02gridmanagement}. 
GridRPC~\cite{seymour02gridrpc} defines an API for executing 
functions on remote servers requiring that developers implement
the client and the server code. 
\name{} extends these ideas to allow interpreted functions
to be registered and subsequently to be dynamically 
executed within sandboxed containers via a standard endpoint API.


Container orchestration systems~\cite{rodriguez19containers, hightower17kubernetes, hindman11mesos} allow
users to scale deployment of containers while 
managing scheduling, fault tolerance, resource provisioning, and addressing
other user requirements. 
These systems primarily rely on dedicated, cloud-like
infrastructure and cannot be directly applied to HPC resources. 
However, these tools provide a basis for other serverless platforms, such as Knative~\cite{knative} and Kubeless~\cite{kubeless}. Knative is a middleware that simplifies deploying serverless applications on a variety of resources using Kubernetes and public clouds.
\name{} 
provides similar functionality, 
however it focuses at the level of scheduling and managing functions, that are deployed
across a pool of containers, rather than deploying services. In addition, it does not rely on container orchestration systems and can interface with almost any computing resource. We apply approaches from container orchestration
systems (e.g., warming) to improve performance.


Data-parallel systems such as Hadoop~\cite{hadoop} and Spark~\cite{spark}
enable map-reduce style analyses. 
Unlike \name{}, these systems dictate a particular programming
model on dedicated clusters. 
Parallel computing libraries such as Dask~\cite{dask}, Parsl~\cite{babuji19parsl}, 
and Ray~\cite{moritz2018ray} support parallel execution of scripts, 
and selected functions within those scripts, 
on clusters and clouds. \name{} uses Parsl to manage
function execution in containers.



